Paraconsistency and Word Puzzles

Word puzzles and the problem of their representations in logic languages have received considerable attention in the last decade (Ponnuru et al. 2004; Shapiro 2011; Baral and Dzifcak 2012; Schwitter 2013). Of special interest is the problem of generating such representations directly from natural language (NL) or controlled natural language (CNL). An interesting variation of this problem, and to the best of our knowledge, scarcely explored variation in this context, is when the input information is inconsistent. In such situations, the existing encodings of word puzzles produce inconsistent representations and break down. In this paper, we bring the well-known type of paraconsistent logics, called Annotated Predicate Calculus (APC) (Kifer and Lozinskii 1992), to bear on the problem. We introduce a new kind of non-monotonic semantics for APC, called consistency preferred stable models and argue that it makes APC into a suitable platform for dealing with inconsistency in word puzzles and, more generally, in NL sentences. We also devise a number of general principles to help the user choose among the different representations of NL sentences, which might seem equivalent but, in fact, behave differently when inconsistent information is taken into account. These principles can be incorporated into existing CNL translators, such as Attempto Controlled English (ACE) (Fuchs et al. 2008) and PENG Light (White and Schwitter 2009). Finally, we show that APC with the consistency preferred stable model semantics can be equivalently embedded in ASP with preferences over stable models, and we use this embedding to implement this version of APC in Clingo (Gebser et al. 2011) and its Asprin add-on (Brewka et al. 2015).

==> jobs_puzzle.tex <==
\section{The Jobs Puzzle in APC and Experiments} \label{jobsPuzzle}

Sentence 1-3 are simples sentences describing the facts of person and gender.

\begin{enumerate}
    \item[1] Roberta is a person. Thelma is a person. Steve is a person. Pete is a person.
    \item[] truth(person(roberta),t).truth(person(thelma),t).truth(person(steve),t).\\truth(person(pete),t).
    \item[2] Roberta is female. Thelma is female.
    \item[] truth(female(roberta),t). truth(female(thelma),t).
    \item[3] Steve is male. Pete is male.
    \item[] truth(male(steve),t). truth(male(pete),t).
\end{enumerate}

We rephrase sentence 4, ``Exclude that a person is male and that the person is female,'' in Schwitter's translation as a sentence of pattern i. The encoding is based on principle 2.
\begin{enumerate}
\item[4] A person is either male or female.
\item[] truth(male(X),t);truth(female(X),t):-truth(person(X),t).
\item[] truth(male(X),f);truth(female(X),f):-truth(person(X),t).
\item[] truth(female(X),top):-truth(person(X),t),truth(male(X),top).
\item[] truth(male(X),top):-truth(person(X),t),truth(female(X),top).
\end{enumerate}

The encoding of sentence 5-6 is based on principle 1. For sentence 5, the first rule forces a job to be hold by exactly one person. The second rule applies the closed world assumption to ensure the complete knowledge of a person holding a job. For sentence 6, the first rule forces a person to hold exactly two jobs. We also apply the closed world assumption to sentence 6. It has the same representation as sentence 5, and therefore eliminated.
\begin{enumerate}
\item[5] If there is a job then exactly one person holds the job.
\item[] 1 \{truth(hold(X,Y),t):truth(person(X),t)\} 1:-truth(job(Y),t).
\item[] truth(hold(X,Y),f):-truth(person(X),t),truth(job(Y),t),not truth(hold(X,Y),t).
\item[6] If there is a person then the person holds exactly two jobs.
\item[] 2 \{truth(hold(X,Y),t):truth(job(Y),t)\} 2:-truth(person(X),t). 
\end{enumerate}

Sentence 7 are simple sentences stating the facts about jobs. 
\begin{enumerate}
\item[7] Chef is a job. Guard is a job. Nurse is a job. Operator is a job. Police is a job. Teacher is a job. Actor is a job. Boxer is a job.
\item[] truth(job(chef),t). truth(job(guard),t). truth(job(nurse),t). truth(job(operator),t).\\ truth(job(police),t). truth(job(teacher),t). truth(job(actor),t). truth(job(boxer),t).
\end{enumerate}

Sentence 8-12 are encoded based on Principle 4, therefore inhibiting deriving inconsistency with respect to job and person.
\begin{enumerate}
\item[8] If a person holds a job as nurse then the person is male.
\item[] truth(male(X),t);truth(hold(X,nurse),f):-truth(person(X),t),truth(job(nurse),t),\par
\qquad \qquad \qquad \qquad \qquad \qquad \qquad \quad  not truth(person(X),top),not truth(job(nurse),top).
\item[9] If a person holds a job as actor then the person is male.
\item[] truth(male(X),t);truth(hold(X,actor),f):-truth(person(X),t),truth(job(actor),t),\par \qquad \qquad \qquad \qquad \qquad \qquad \qquad \quad not truth(person(X),top),not truth(job(actor),top).
\item[10] If a first person holds a job as chef and a second person holds a job as telephone operator then the second person is a husband of the first person.
\item[] truth(husband(Y,X),t);truth(hold(X,chef),f);truth(hold(Y,operator),f):-\par \quad \qquad truth(person(X),t),truth(job(chef),t),truth(person(Y),t),truth(job(operator),t),\par \qquad \qquad not truth(person(X),top),not truth(job(chef),top),\par \qquad \qquad not truth(person(Y),top),not truth(job(operator),top).
\item[11] If a first person is a husband of a second person then the first person is male.
\item[] truth(male(X),t);truth(husband(X,Y),f):-truth(person(X),t),truth(person(Y),t),\par \qquad \qquad \qquad \qquad \qquad \qquad \qquad \quad not truth(person(X),top),not truth(person(Y),top).
\item[12] If a first person is a husband of a second person then the second person is female.
\item[] truth(female(Y),t);truth(husband(X,Y),f):-truth(person(X),t),truth(person(Y),t),\par \qquad \qquad \qquad \qquad \qquad \qquad \qquad \quad not truth(person(X),top),not truth(person(Y),top).
\end{enumerate}

Sentence 13 and 14 are \textbf{Exclude\ that} sentences. We encode sentence 13 based on principle 4 and encode sentence 14 as a single predicate annotated as \textbf{f}.
\begin{enumerate}
\item[13] Exclude that Roberta holds a job as boxer.
\item[] truth(hold(roberta,boxer),f):-truth(job(boxer),t),not truth(job(boxer),top).
\item[14] Exclude that Pete is educated.
\item[] truth(educated(pete),f).
\end{enumerate}

For the rest, sentence 15-17 are encoded based on principle 4. Sentence 18-20 are encoded in a similar way as sentence 13-14.
\begin{enumerate}
\item[15] If a person holds a job as nurse then the person is educated.
\item[] truth(educated(X),t);truth(hold(X,nurse),f):-truth(person(X),t),truth(job(nurse),t), \par \qquad \qquad \qquad \qquad \qquad \qquad \qquad \quad not truth(person(X),top),not truth(job(nurse),top).
\item[16] If a person holds a job as police officer then the person is educated.
\item[] truth(educated(X),t);truth(hold(X,police),f):-truth(person(X),t),truth(job(police),t),\par \qquad \qquad \qquad \qquad \qquad \qquad \qquad \quad not truth(person(X),top),not truth(job(police),top).
\item[17] If a person holds a job as teacher then the person is educated.
\item[] truth(educated(X),t);truth(hold(X,teacher),f):-truth(person(X),t),truth(job(teacher),t),\par \qquad \qquad \qquad \qquad \qquad \qquad \qquad not truth(person(X),top),not truth(job(teacher),top).
\item[18] Exclude that Roberta holds a job as chef.
\item[] truth(hold(roberta,chef),f):-truth(job(chef),t),not truth(job(chef),top).
\item[19] Exclude that Roberta holds a job as police officer.
\item[] truth(hold(roberta,police),f):-truth(job(police),t),not truth(job(police),top).
\item[20] Exclude that a person holds a job as chef and that the person holds a job as police officer.
\item[] truth(hold(X,chef),f);truth(hold(X,police),f):-truth(person(X),t),truth(job(chef),t),\par \qquad \qquad \qquad \qquad \qquad \qquad truth(job(police),t), not truth(person(X),top),\par \qquad \qquad \qquad \qquad \qquad \qquad not truth(job(chef),top),not truth(job(police),top).
\end{enumerate}

Before describing the preference relations, we first give the specifications of the domain and the herbrand universe of the puzzle.
\begin{enumerate}
\item[] dom(roberta;thelma;steve;pete;chef;guard;nurse;operator;police;teacher;actor;boxer).
\item[] hu(person(X)):-dom(X).
\item[] hu(job(X)):-dom(X).
\item[] hu(hold(X,Y)):-dom(X),dom(Y).
\item[] hu(male(X)):-dom(X).
\item[] hu(female(X)):-dom(X).
\item[] hu(husband(X,Y)):-dom(X),dom(Y).
\item[] hu(educated(X)):-dom(X).
\end{enumerate}

The preference relations are specified below:
\begin{enumerate}
\item[] $\#$preference(all,lexico)\{3$::$name(p3);2$::$name(p2);1$::$name(p1)\}.
\item[] $\#$preference(p3,subset)\{ truth(person(X),top) : dom(X);truth(job(Y),top) : dom(Y)\}.
\item[] $\#$preference(p2,subset)\{ truth(X,top) : hu(X)\}.
\item[] $\#$preference(p1,poset)\{ hp(X,bottom)$>$hp(X,f):hu(X); hp(X,f)$>$hp(X,t):hu(X);\par \qquad \qquad \qquad \qquad \qquad hp(X,t)$>$hp(X,top):hu(X)\}.
\item[] $\#$optimize(all).
\end{enumerate}

Preference \textit{p3} says that we prefer models with minimal inconsistency with respect to person and job. Preference \textit{p2} says that we prefer models with minimal inconsistency. Preference \textit{p1} specifies the partial order among $\perp$, $\textbf{t}$, $\textbf{f}$, and $\top$. That is, $\perp>\textbf{t}>\textbf{f}>\top$, where $a>b$ says that $a$ is preferred over $b$. Preference \textit{p3} says that we prefer models with a maximal set of $\perp$-predicates. Among the models with a maximal set of $\perp$-predicates, we prefer the one with a maximal set of $\textbf{f}$-predicates. The same applies to $\textbf{t}$-predicates and $\top$-predicates. Preference $\textit{p1}$, $\textit{p2}$, and $\textit{p3}$ are combined by the \textit{lexico} relation. In a high level, the first statement says that we first minimize \textit{p3}, then minimize \textit{p2}, and finally minimize \textit{p1}.

The above encoding generates the same answer as the original Jobs Puzzle's:
\begin{enumerate}
\item[] truth(hold(pete,actor),t) 
\item[] truth(hold(pete,operator),t) 
\item[] truth(hold(steve,police),t) 
\item[] truth(hold(steve,nurse),t)
\item[] truth(hold(thelma,chef),t)
\item[] truth(hold(thelma,boxer),t)
\item[] truth(hold(roberta,guard),t)
\item[] truth(hold(roberta,teacher),t)
\end{enumerate}

Next, we show how APC handles inconsistency by adding three sentences separately to the original puzzle.  
\begin{enumerate}
\item[21] Thelma is an actor
\item[] truth(hold(thelma,actor),t).
\end{enumerate}
There are two answers:
\begin{enumerate}
\item[] Answer 1:
\item[] truth(hold(pete,boxer),t) truth(hold(pete,operator),t) truth(hold(steve,police),t) \par truth(hold(steve,nurse),t) truth(hold(thelma,actor),top)  truth(hold(thelma,chef),t) \par truth(hold(roberta,teacher),t) truth(hold(roberta,guard),t) truth(husband(pete,thelma),t)
\end{enumerate}
\begin{enumerate} 
\item[] Answer 2:
\item[]  truth(hold(pete,boxer),t) truth(hold(pete,operator),t) truth(hold(steve,police),t) \par truth(hold(steve,nurse),t) truth(hold(thelma,actor),t) truth(hold(thelma,chef),t) \par truth(hold(roberta,teacher),t) truth(hold(roberta,guard),t) truth(female(thelma),top) \par truth(male(thelma),top) truth(husband(pete,thelma),t)
\end{enumerate}
Given that the puzzle implicitly implies that Thelma is not supposed to hold a job of actor, sentence 21 will cause an inconsistency. In the first case, we refute sentence, and therefore generating an inconsistency with respect to Thelma holding a job of actor. In the second case, we accept sentence 21 as a valid statement. Based on sentence 4, we infer that Thelma is both male and female, therefore generating inconsistency with respect to Thelma's gender. 

\begin{enumerate}
\item[22] Steve is female.
\end{enumerate}
There are two answers:
\begin{enumerate}
\item[] Answer 1:
\item[] truth(hold(pete,actor),t) truth(hold(pete,operator),t) truth(hold(steve,police),t) \par truth(hold(steve,nurse),t) truth(hold(roberta,teacher),t) truth(hold(thelma,boxer),t) \par truth(hold(roberta,guard),t) truth(hold(thelma,chef),t)  h(husband(pete,thelma),t) \par truth(male(steve),top) truth(female(steve),top)
\end{enumerate}
\begin{enumerate}
\item[] Answer 2:
\item[] truth(hold(pete,actor),t) truth(hold(pete,operator),t) truth(hold(steve,nurse),t)  \par truth(hold(steve,chef),t) truth(hold(thelma,boxer),t) truth(hold(thelma,police),t) \par truth(hold(roberta,guard),t) truth(hold(roberta,teacher),t) truth(husband(pete,steve),t) \par truth(female(steve),top) truth(male(steve),top)
\end{enumerate}
Given that Steve is male, sentence 22 will cause an inconsistency with respect to Steve's gender. The first answer is the same as the original  puzzle's except for the inconsistency with respect to Steve's gender. Since Steve is also considered as female, the second answer considers Pete as Steve's husband and therefore deriving that Steve holds a job of chef.

\begin{enumerate}
\item[23] Steve is a husband of Thelma.
\end{enumerate}
Since the original translation does not indicate the implicit knowledge that a person has at most one husband or a person is at most one person's husband, adding the above sentence will not change the answer to the puzzle except that Thelma has two husbands. To make this implicit knowledge explicit, we add two additional sentences:
\begin{enumerate}
\item[24] A person has at most one husband.
\item[25] A person is at most one person's husband.
\end{enumerate}

\begin{enumerate}
\item[] {truth(husband(X,Y),t):truth(person(Y),t)} 1:-truth(person(X),t).
\item[] truth(husband(X,Y),f):-truth(person(X),t),truth(person(Y),t),not truth(husband(X,Y),t).
\item[] {truth(husband(X,Y),t):truth(person(X),t)} 1:-truth(person(Y),t).
\end{enumerate}

Given that one person has at most one husband and that Steve is Thelma's husband, Pete will not be inferred as Thelma's husband, and therefore generating inconsistency to  the puzzle.

%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "main"
%%% End: 

